Logic Blog 2019

The blog focusses on algorithmic randomness and its connections to quantum information theory, group theory and its connections to logic, and computability analogs of cardinal characteristics.

==> sections2019/Nies_MAD_high__Santiago_Figueira_s_conflicted_copy_2019-12-04_.tex <==
\section{Nies: potential computability analogs of cardinal invariants not given by relations}

The following ideas resulted from some interactions of Nies with Brendle, Greenberg and others  at the August meeting on set theory of the reals  at Casa Matem\'atica Oaxaca, which was  organised by Hrusak, Brendle, and Steprans. 

Let $\frb$  be the unbounding number (least size of a class of functions on $\omega$ that is not dominated by a single function). 

Several cardinal characteristics are based on cardinals  of subclasses of $\+ P(\omega)/{=^*} \setminus \{0\}$, i.e. the infinite sets under almost inclusion.  One of them is   $\mathfrak a$,  called the almost disjointness number, which is  the minimal size of a maximal almost disjoint (MAD) family of subsets of $\omega$. 
It is well known  that

\begin{fact}  \label{fa: ba} $\frb \le \mathfrak a$. \end{fact}

The analog of $\frb$ is the  property of oracles $C$ to be   high, namely  $\ES'' \le_T C'$; for detail  on this see~\cite{Rupprecht:10,Brendle.Brooke.ea:14}.  We want to introduce a possible analog $\+ A$ of $\mathfrak a$,  and show that the analogous relationship holds: every high oracle computes a set in $\+ A$.  (The inversion here is part of the generally accepted setup of translation between the two areas of logic.)

\begin{proof}[Proof  of Fact~\ref{fa: ba}] Suppose that the infinite cardinal $\kappa$ is less than $\frb$. Let $\+ V$ be an almost disjoint family of size  $\kappa$. We show that $\+ V$ is not MAD. Let $\seq {r_n}$, $n \in \omega$,  be a sequence of pairwise distinct elements of $\+ V$. Given $y \in \+ V$ let \bc $f_y(n) = \max  (y \cap r_n)$ \ec
with the convention that $\max \ES = 0$. Let $g$ be an increasing  function such that $g(n) \in r_n$ for each $n$  and $\forall y \in \+ V \forall^\infty n  \, [ g(n) > f_y(n)]$.  It is clear that the family $\+ V \cup \{\range (g)\}$ is almost disjoint.  \end{proof}


Other  cardinal characteristics are based on properties   of subclasses of  the infinite sets under almost inclusion: 
\bi \item  the ultrafilter number $\fru$ (the least size of a set  with upward closure  a free ultrafilter on $\omega$), \item the  tower number $\mathfrak t$ (the minimum size of a   linearly ordered subset that can't be extended by putting a new element below), \item the  independence number $\mathfrak i$  \ei  and several others. See e.g.\ \cite{Blass:10} or the  talk by Diana Montoya at the CIRM meeting on descriptive set theory in June 2018, which contains a Hasse diagram of these cardinals with ZFC inequalities, reproduced here with permission: 


\bc \includegraphics[width=2.5in]{sections2019/Montoya_Hasse_diagram} \ec

Note that $\mathfrak r$ and $\mathfrak s$ are the unreaping and splitting numbers, respectively. They are given by relations, and their analogs have been studied \cite{Brendle.Brooke.ea:14}. Furthermore,  $\mathfrak e$ is the escaping number (Brendle and Shelah, recently studied in computability theory by Ongay Valverde and Tveite), and $\mathfrak h$ is the distributivity number.  

A uniform way to translate these characteristics into highness properties  of oracles in computability is  as follows. 
Consider analogous properties for subclasses of $\+ P(\text{Rec})/{=^*} \setminus \{0\}$, identified with classes of   infinite recursive sets in the context of  almost inclusion.    A subclass $\+ C$  is encoded by a set $F$ such that \bc $\+ C = \+ C_F =   \{F^{[n]} \colon n \in \NN\}$, \ec where $F^{[n]}$ is  column $\{ x \colon \la x, n \ra \in F\}$. 

\begin{definition} The highness property $\+ A$  corresponding to the almost disjointness number $\fra$ is the class of oracles that compute a set $F$  such that $\+ C_F$ is MAD within the recursive sets. Namely, $\+ C_F$ is almost disjoint, and  for each infinite recursive set $R$ there is $B \in \+ C_F$ such that $R\cap B $ is infinite. \end{definition}

\begin{definition} The highness property $\+ U$  corresponding to the ultrafilter  number $\fru$ is the class of oracles that compute a set $F$  such that $\+ C_F$ is an ultrafilter base within the recursive sets. Namely, each finite intersection of elements of $\+ C_F$ is infinite, and  for each infinite recursive set $R$ there is $B \in \+ C_F$ such that $B \sub^* R$ or $ B \cup R $ is cofinite. \end{definition}

Since the  properties of (codes for) classes are arithmetical, each of those highness property contains $\ES^{(n)}$ for sufficiently large $n$. For instance, to see that $\ES^{(2)} \in \+ U$, take any $r$-maximal set $C$. By definition  the recursive sets $R$ such that $R \cup C$ is cofinite form an ultrafilter. We can encode it as $\+ C_F$ for some $F \le_T \ES''$. 

Analog of $\frb \le \fra$.
\begin{theorem} Each high oracle  $C$  is in $\+ A$. \end{theorem}



 

==> sections2019/Nies_Stephan_almost_abelian.tex <==
\section{Nies and Stephan: Some properties of \\ infinitely generated nilpotent-of-class-2 groups}


\subsection{Three properties of an elementary abelian group} Throughout fix a prime $p$. Let $G= F_p^{(\omega)}$ denote the elementary abelian $p$ group (i.e., vector space over  the field $F_p$ of infinite dimension). This group has the following apparently unrelated properties.

\begin{definition}  \mbox{} 
\begin{enumerate}  \item $G$ is word-automatic in the usual sense of Khoussainov and Nerode: it has a representation on strings over a finite alphabet such that  finite automata can recognize the domain and the group operations.

\item $G$ is $\omega$-categorical: it is  up to isomorphism the only countable model of its theory.
\item $G$ is pseudofinite: if a sentence $\phi$ holds in $G$ then $\phi$ also holds in a finite group.  \end{enumerate}
\end{definition}
Note that a word automatic group is called \emph{finite automata presentable} in Nies~\cite{Nies:DescribeGroups}  in order to avoid confounding the notion   with the better known notion of automatic groups due to Thurston.   The group $F_p^{(\omega)}$ is $\omega$-categorical because for each $n$ there are only finitely many $n$-types.  To show that $F_p^{(\omega)}$  is pseudofinite, note that its theory is axiomatized by stating that the group is infinite,  has exponent $p$ and is abelian. So we may assume that $\phi$ is a finite conjunction of these axioms, which clearly has a finite model. 

\subsection{Groups that are nilpotent of class 2}
Usually we will assume  that  $p\neq 2$.
We want to study the three properties above for groups that are very close to abelian. Recall that a group  $G$ is \emph{nilpotent  of class 2} if each commutator $[x,y]$ is in the centre $C(G)$. In other words, $G$ is an extension of a group $N$ by a group $Q$ that is  abelian,  and $N $ is   contained in $C(G)$ (i.e., a central extension). It is not hard to show that such a group is entirely given by the abelian groups $N$, $Q$, and an alternating  bilinear map $L \colon \,  Q \times Q  \to N$. It determines a unique central extension $G$  such that $L(Nx,Ny) = [x,y]$ (note that $[x,y] $ only depends on the cosets of $x,y$).  In fact this is a special case of the well known fact that an extension of abelian group $N$ by $Q$  is given by an element of the second co-homology group $H^2(Q,N)$. 

We will study our properties for  three  examples of infinitely generated groups of exponent $p$.  We will always have $Q =F_p^{(\omega)}$,   and fix  a basis $\seq {x_i}\sN i$  of $Q$.

  Let $L_p$ be the free nilpotent-2 exponent $p$ group  of infinite rank. One  has $N\cong Q$;  let $y_{i,k}$ ($i< k$) be free generators of $N$. It is given by the function $\phi (x_i, x_k) = y_{i,k}$ if $i<k$.  Thus 
  
  \bc $L_p = \la x_i, y_{i,k} \mid x_i^p, [x_i, x_k] y_{i,k}^{-1} , [y_{i,k}, x_r] (i< k) \ra$ \ec
where the $y_{i,k}$ are actually redundant.


$G_p$ is the group where $Q = F_p^{(\omega)}$, $N = C_p$ (cyclic group of order $p$)  and   $\phi (x_i, x_k) = 1$ if $i<k$, $-1$ if $i > k$ (and of course $0$ if $i=k$). So 

\bc $G_p = \la x_i, u \mid x_i^p, [x_i, x_k] u^{-1} , [u, x_r]   \,  (i< k, 0 \le r) \ra $. \ec


The group $H_p$ has $N \cong Q$, with  free generators $z_k$ ($k >0$), and the function $\phi (x_i, x_k) = z_k$ if $i<k$:

\bc $H_p = \la x_i, z_{k} \mid x_i^p, [x_i, x_k] z_{k}^{-1} , [z_{k}, x_r] \,  (i< k, 0 \le r) \ra $. \ec


\subsection{FA-presentability}
Any FA presentable structure has a decidable theory. Ershov~\cite{Ershov:72} showed  that a finitely generated nilpotent group has decidable first-order theory if and only if it is virtually abelian. 
 One the other hand, \cite[Thm.\ 4.2]{Nies.Semukhin:09} showed that  an abelian group that is extension of finite index of an FA-presentable group is in itself FA-presentable. So a f.g.\ nilpotent group is FA-presentable iff it is abelian by finite.
 Thus, only in the infinitely generated case interesting things can happen. 


 
\begin{fact} $G_p$ is FA-presentable. \end{fact}


\begin{proof}  Each element has the form $c \cdot q$ where $c \in N$, $q\in Q$. 
 Note that   $q$ is given as a string $\alpha$ over the alphabet  of digits $0, \ldots, p-1$, and $c$ can be stored in the state. In the following $\alpha, \beta$ denote such strings, which are thought of as extended by $0$'s if necessary. Let $[\alpha] = \prod_i x_i^{\alpha_i}$. It is easy to verify that using arithmetic modulo $p$, and component-wise addition of strings
 
 \[ [\alpha] [\beta] =  [\alpha + \beta] u^{\sum_{k>0}\alpha_k (\sum_{i< k} \beta_i}).\]
 This is because   in calculating $\prod_k x_k^{\alpha_k} \prod_i x_i^{\beta_i}$ for decreasing positive $k$ we   move   $x_k^{\alpha_k}$ past the $x_i^{\beta_i}$ for $i=0, \ldots, k-1$, and each such move creates a factor $u^{\alpha_k \beta_i}$.  A finite automaton processing $\alpha, \beta $ on two tracks can remember the current $\sum_{i< k} \beta_i$ in the state, and also carry out the calculation $\alpha_k (\sum_{i< k} \beta_i)$ and store the current exponent of $u$ in the state.
  \end{proof}
%  Note that $G_p$ has an abelian  subgroup $B$ of finite index isomorphic to $F_p^{(\omega)}$:  let $B $ be the kernel of the map $G_p \to C_p$ that maps an element $cq$ to the exponent of $x_0$ in $q$. So the result follows from

\begin{fact} $H_p$ is FA-presentable. \end{fact}


Frank please add. How about $L_p$? probably not....

